Improving Weakly-Supervised Object Localization Using Adversarial Erasing and Pseudo Label

Weakly-supervised learning approaches have gained significant attention due to their ability to reduce the effort required for human annotations in training neural networks. This paper investigates a framework for weakly-supervised object localization, which aims to train a neural network capable of predicting both the object class and its location using only images and their image-level class labels. The proposed framework consists of a shared feature extractor, a classifier, and a localizer. The localizer predicts pixel-level class probabilities, while the classifier predicts the object class at the image level. Since image-level class labels are insufficient for training the localizer, weakly-supervised object localization methods often encounter challenges in accurately localizing the entire object region. To address this issue, the proposed method incorporates adversarial erasing and pseudo labels to improve localization accuracy. Specifically, novel losses are designed to utilize adversarially erased foreground features and adversarially erased feature maps, reducing dependence on the most discriminative region. Additionally, the proposed method employs pseudo labels to suppress activation values in the background while increasing them in the foreground. The proposed method is applied to two backbone networks (MobileNetV1 and InceptionV3) and is evaluated on three publicly available datasets (ILSVRC-2012, CUB-200-2011, and PASCAL VOC 2012). The experimental results demonstrate that the proposed method outperforms previous state-of-the-art methods across all evaluated metrics.

==> sections/tbl_result_ablation.tex <==

\begin{table*}[!t]
\begin{center}
\begin{minipage}{0.95\linewidth}
\caption{Ablation study on loss terms using the MobileNetV1 backbone~\citep{mobilenetv1} and the CUB-200-2011 dataset~\citep{cub_dataset}.}
\label{tab:result_ablation1}
\renewcommand{\arraystretch}{1.1} 
\begin{tabu}{X[c,m]|X[c,m]|X[c,m]|X[c,m]|X[c,m]|X[c,m]|X[c,m]} 
\hline
\multicolumn{4}{c|}{Method} & \multirow{2}{*}{Top-1} & \multirow{2}{*}{Top-5} & \multirow{2}{*}{GT-known}  \\ 
\tabucline{1-4}
Baseline & $\calL_{pseudo}$ & $\calL_{ae\text{-}fg}$ & $\calL_{ae}$ & & & \\ 
\hline\hline
\checkmark & $-$ & $-$ & $-$ & 69.77 & 86.00 & 92.35 \\
\checkmark & \checkmark & $-$ & $-$ & 70.41 & 86.07 & 92.48 \\
\checkmark & \checkmark & \checkmark & $-$ & 70.46 & 86.71 & 92.83  \\
\checkmark & \checkmark & \checkmark & \checkmark & \textbf{71.28}& \textbf{87.00}&\textbf{93.03} \\
\hline  		
\end{tabu}
\end{minipage}
\end{center}
\end{table*}



\begin{table*}[!t]
\begin{center}
\begin{minipage}{0.95\linewidth}
\caption{Ablation study on weighting coefficients in the total loss by using the MobileNetV1 backbone~\citep{mobilenetv1} and the CUB-200-2011 dataset~\citep{cub_dataset}.}
\label{tab:result_ablation2}
\renewcommand{\arraystretch}{1.1} 
\begin{tabu}{X[c,m]|X[c,m]|X[c,m]|X[c,m]|X[c,m]|X[c,m]|X[c,m]|X[c,m]|X[c,m]} 
\hline
\multicolumn{6}{c|}{Weighting coefficients} & \multirow{2}{*}{Top-1} & \multirow{2}{*}{Top-5} & \multirow{2}{*}{GT-known}  \\ 
\tabucline{1-6}
$\gamma_1$ & $\gamma_2$ & $\gamma_3$ & $\gamma_4$ & $\gamma_5$ & $\gamma_6$ & & & \\ 
\hline\hline
\checkmark & $-$ & $-$ & $-$ & 69.77 & 86.00 & 92.35 \\
\checkmark & \checkmark & $-$ & $-$ & 70.41 & 86.07 & 92.48 \\
\checkmark & \checkmark & \checkmark & $-$ & 70.46 & 86.71 & 92.83  \\
\checkmark & \checkmark & \checkmark & \checkmark & \textbf{71.28}& \textbf{87.00}&\textbf{93.03} \\
\hline  		
\end{tabu}
\end{minipage}
\end{center}
\end{table*}




==> sections/tbl_result_inception.tex <==
\begin{table*}[!t]
\centering
\begin{minipage}{0.95\linewidth}
\caption{Quantitative results of the methods using InceptionV3 as the backbone.}
\label{tab:result_inception}
\renewcommand{\arraystretch}{1.1} 
\begin{tabular}{ >{\centering}m{0.25\textwidth}| >{\centering}m{0.13\textwidth}| *{5}{>{\centering}m{0.07\textwidth}|} >{\centering\arraybackslash}m{0.07\textwidth} } 
\hline
\multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c}{ILSVRC} \\ 
\cline{3-8}
 &  &  Top-1 & Top-5 & GT-known & Top-1 & Top-5 & GT-known \\ 
\hline\hline
CAM~\citep{cam2016} & 
& 41.06 & 50.66 & 55.10  &  46.29 & 58.19 & 62.68 \\
SPG~\citep{spg2018} & 
& 46.64 & 57.72 & -  & 48.60 & 60.00 & 64.69 \\
DANet~\citep{Xue2019} & 
& 49.45 & 60.46 & 67.03  & 47.53 & 58.28 & - \\
PSOL~\citep{Zhang2020} & 
&  65.51 & 83.44 & -  &  54.82 & 63.25 & 65.21 \\
I2C~\citep{i2c2020} & 
& 55.99 & 68.34 & 72.60  & 53.11 & 64.13 & 68.50 \\
GCNet~\citep{Lu2020} & InceptionV3
& 58.58 & 71.00 & 75.30  & 49.06 & 58.09 & - \\
RCAM~\citep{Bae2020} & 
& 53.04 & - & 69.95  & 50.56 & - & 64.44 \\
SPA~\citep{Pan2021} & 
& 53.59 & 66.50 & 72.14  & 52.73 & 64.27 & 68.33 \\
SLT~\citep{Guo2021} & 
&  66.10 & - & 86.50  &  55.70 & 65.40 & 67.60 \\
FAM~\citep{Meng2021} & 
& 70.67 & - & 87.25  & 55.24 & - &68.62\\
BAS~\citep{Wu_2022_CVPR} & 
&\underline{73.29}&\underline{86.31}&\underline{92.24} &\underline{58.51}&\underline{69.00}&\underline{71.93}\\
Proposed & 
& \textbf{73.79}& \textbf{87.99}&\textbf{94.08} & \textbf{58.85}& \textbf{69.50}&\textbf{72.52}\\
\hline  
\end{tabular}
\end{minipage}
\end{table*}



==> sections/tbl_result_mobilenet.tex <==
\begin{table*}[!t]
\centering
\begin{minipage}{0.95\linewidth}
\caption{Quantitative results of the methods using MobileNetV1 as the backbone.}
\label{tab:result_mobilenet}
\renewcommand{\arraystretch}{1.1} 
\begin{tabular}{ >{\centering}m{0.25\textwidth}| >{\centering}m{0.13\textwidth}| *{5}{>{\centering}m{0.07\textwidth}|} >{\centering\arraybackslash}m{0.07\textwidth} } 
\hline
\multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c}{ILSVRC} \\ 
\cline{3-8}
 &  &  Top-1 & Top-5 & GT-known & Top-1 & Top-5 & GT-known \\ 
\hline\hline
CAM~\citep{cam2016} & 
& 48.07 & 59.20 & 63.30 & 43.35 & 54.44 & 58.97 \\
HaS~\citep{hideseek2017} & 
& 46.70 & - & 67.31  & 42.73 & - & 60.12 \\
ADL~\citep{Choe2019} & 
& 47.74 & - & -  & 43.01 & - & - \\
RCAM~\citep{Bae2020} & MobileNetV1
& 59.41 & - & 78.60  & 44.78 & - & 61.69 \\
FAM~\citep{Meng2021} & 
& 65.67 & - & 85.71  & 46.24 & - & 62.05 \\
BAS~\citep{Wu_2022_CVPR} & 
& \underline{69.77}& \underline{86.00}&\underline{92.35} & \underline{52.97}& \underline{66.59}&\underline{72.00}\\
Proposed & 
& \textbf{71.28}& \textbf{87.00}&\textbf{93.03} & \textbf{53.68}& \textbf{67.07} & \textbf{72.18}\\
\hline  		
\end{tabular}
\end{minipage}
\end{table*}



